Physical Modeling using Recurrent Neural Networks with Fast Convolutional Layers

Discrete-time modeling of acoustic, mechanical and electrical systems is a prominent topic in the musical signal processing literature. Such models are mostly derived by discretizing a mathematical model, given in terms of ordinary or partial differential equations, using established techniques. Recent work has applied the techniques of machine-learning to construct such models automatically from data for the case of systems which have lumped states described by scalar values, such as electrical circuits. In this work, we examine how similar techniques are able to construct models of systems which have spatially distributed rather than lumped states. We describe several novel recurrent neural network structures, and show how they can be thought of as an extension of modal techniques. As a proof of concept, we generate synthetic data for three physical systems and show that the proposed network structures can be trained with this data to reproduce the behavior of these systems.

==> ftm.tex <==
The FTM is a powerful method for modeling the oscillation of acoustic systems in terms of transfer functions and a detailed description of its derivation and application can be found, e.g., in \cite{Trautmann2003DigitalMethod, Schafer2019SimulationModels,petrausch:SMMSP:2004}. For example, the method has been applied for the modeling of strings (see, e.g., \cite{schaefer:dafx:2016,trautmann:2003b}), membranes (see, e.g., \cite{rabenstein:ieee:2010,Schafer2019FeedbackMembrane,Han2020}, and room acoustics (see, e.g., \cite{Petrausch2005SimulationMethod,Schafer2020ASynthesis}).
The basic idea of the FTM is to transform the mathematical description of an acoustical system in terms of PDEs into a discrete-time simulation model by the application of functional transformations for time and space dependencies. In the following we present the most essential steps of the FTM necessary for the application to the considered acoustical system and to highlight the relation to the proposed NN structure.

\subsection{FTM Modeling Procedure}
The application of the FTM starts from an initial-boundary-value problem in the form of a unifying vector formulation \cite{petrausch:SMMSP:2004}
\begin{align}
    \left(\mathbf{C}\frac{\partial}{\partial t} - \mathbf{L}\right)\mathbf{u}(\mathbf{x},t) &= 0, &\mathbf{x}\in V, \, t > 0,\label{eq:ftm:1}\\
    \mathbf{F}_\mathrm{b}\her\mathbf{u}(\mathbf{x},t) &= \bm{\phi}(t), &\mathbf{x}\in\partial V, \, t > 0,\label{eq:ftm:2}\\
    \mathbf{u}(\mathbf{x},t) &= \mathbf{u}_\mathrm{i}(\mathbf{x}), &\mathbf{x}\in V, \, t = 0,
    \label{eq:ftm:3}
\end{align}
defined on spatial domain $V$ and its boundary $\partial V$. In PDE \eqref{eq:ftm:1}, matrix $\mathbf{C}\in\mathbb{R}^{N\times N}$ is a capacitance matrix and $\mathbf{L}$ is a $N\times N$ sized spatial differentiation operator. 
The state vector $\mathbf{u}\in\mathbb{R}^{N\times 1}$ contains $N$ physical quantities of the underlying acoustical system such as deflection, sound pressure or particle velocities (see, e.g., \cite[Eqs.~(26), (34)]{Schafer2020ASynthesis}). 
Boundary conditions \eqref{eq:ftm:2} are defined in terms of an operator $\mathbf{F}_\mathrm{b}\her\in\mathbb{R}^{N\times N}$ applied to $\mathbf{u}$ yielding the boundary values $\bm{\phi}$. 
We consider homogeneous boundary conditions, $\bm{\phi} = \mathbf{0}$ for all the following example systems. The temporal initial state of the system is modeled by a vector of initial conditions (ICs) $\mathbf{u}_\mathrm{i}\in\mathbb{R}^{N\times 1}$ in~\eqref{eq:ftm:3}. 

In order to derive a FTM model for the system \eqref{eq:ftm:1}-\eqref{eq:ftm:2}, $\mathbf{u}$ is expanded into an infinite set of bi-orthogonal basis functions $\Kprim_\mu\in\mathbb{C}^{N\times 1}$ and $\Kadj_\mu\in\mathbb{C}^{N\times 1}$ for the operator $\mathbf{L}$, where the dedicated eigenvalues $s_\mu$, $\mu\in\mathbb{N}_0$ constitute the discrete spectrum of $\mathbf{L}$ \cite{churchill:1972}. With basis function $\Kprim_\mu$ and $\Kadj_\mu$ a forward and inverse Sturm-Liouville transform (SLT) are defined as follows 
\begin{align}
	\bar{u}_\mu(t) &= \mathcal{T}\{\mathbf{u}(\mathbf{x},t)\} = \int_{V}\Kadj_\mu\her(\mathbf{x})\mathbf{C}\mathbf{u}(\mathbf{x},t)\dint{\mathbf{x}},\label{eq:ftm:4}\\
	\mathbf{u}(\mathbf{x},t) &= \mathcal{T}^{-1}\{\bar{u}_\mu(t)\}=\sum_{\mu = 0}^{\infty} \frac{1}{N_\mu}\bar{u}_\mu(t) \Kprim_\mu(\mathbf{x}). 
	\label{eq:ftm:5}
\end{align}
Forward SLT \eqref{eq:ftm:4} expands $\mathbf{u}$ into the basis functions $\Kadj_\mu$ yielding the expansion coefficients $\bar{u}_\mu$. 
In the context of acoustics, \eqref{eq:ftm:4} expands a system into its modes and the time-dependent expansion coefficients $\bar{u}_\mu$ describe their temporal evolution. 
The inverse SLT in \eqref{eq:ftm:5} represents $\mathbf{u}$ as series expansion with basis functions $\Kprim_\mu$ and scaling factors $N_\mu = \int_V \Kadj_\mu\her\mathbf{C}\Kprim_\mu\dint{\mathbf{x}}$. 
Further properties of \eqref{eq:ftm:4} and \eqref{eq:ftm:5} such as the existence of a differentiation theorem and the bi-orthogonality of $\Kprim$ and $\Kadj$ are discussed in detail in \cite[Sec.~4.7.3]{Schafer2019SimulationModels}.
We note that the shape of $\Kprim$ and $\Kadj$ depends on the spatial shape of the underlying system, e.g., for geometrically simple systems basis functions are often trigonometric functions, Bessel functions or combinations thereof \cite[Sec.~4.7.4]{Schafer2019SimulationModels}. 

Application of the forward SLT \eqref{eq:ftm:4} to PDE \eqref{eq:ftm:1}, exploiting $\bm{\phi}=\mathbf{0}$ and the differentiation theorem \cite[Eq.~(18)]{Schafer2020ASynthesis}, leads to expansion coefficients defined in terms of Laplace transfer functions 
\begin{align}
    &\bar{u}_\mu(t) = \mathrm{e}^{s_\mu t}\bar{u}_{\mathrm{i},\mu} &\laplace && \bar{U}_\mu(s) = \frac{1}{s-s_\mu}\bar{u}_{\mathrm{i},\mu}, 
    \label{eq:ftm:6}
\end{align}
where the coefficients $\bar{u}_{\mathrm{i},\mu}$ follow from the expansion of the initial values $\mathbf{u}_\mathrm{i}$ in \eqref{eq:ftm:3}, i.e.,  $\bar{u}_{\mathrm{i},\mu} = \mathcal{T}\{\mathbf{u}_\mathrm{i}(\mathbf{x})\}$.

Truncating the number of eigenvalues $s_\mu$ to be finite, i.e., $\mu = 0, \dots, Q-1$, and transforming \eqref{eq:ftm:5} and \eqref{eq:ftm:6} into the discrete-time domain allows the formulation of the FTM model in terms of a vector valued state space description (SSD) \cite{Schafer2019SimulationModels,Schafer2019FeedbackMembrane,Schafer2020ASynthesis}
\begin{align}
    \bar{\mathbf{u}}[k+1] &= \mathrm{e}^{\As T}\bar{\mathbf{u}}[k] +T\bar{\mathbf{u}}_\mathrm{i}\delta[k], \label{eq:ftm:7}\\
    \mathbf{u}[\mathbf{x},k] &= \Cs(\mathbf{x})\bar{\mathbf{u}}[k], \label{eq:ftm:8}
\end{align}
with the discrete time index $k$, sampling interval $T$, i.e., $t=kT$, and the discrete-time Dirac delta function $\delta[k]$. \textit{State equation} \eqref{eq:ftm:7} is a vector valued discrete-time version of \eqref{eq:ftm:6}, where the vector $\bar{\mathbf{u}} = \left(\bar{u}_\mu \right)_{\mu = 0}^{Q-1}$ contains the expansion coefficients, the diagonal matrix $\As\in\mathbb{C}^{Q\times Q}$ contains the eigenvalues $s_\mu$ on its main diagonal and $\bar{\mathbf{u}}_\mathrm{i} = \left(\bar{u}_{\mathrm{i},\mu} \right)_{\mu = 0}^{Q-1}$. \textit{Output equation} \eqref{eq:ftm:8} is a clever reformulation of the inverse SLT in \eqref{eq:ftm:5} by representing the truncated sum by a matrix-vector multiplication with the transformation matrix 
\begin{align}
    \Cs(\mathbf{x}) = \left[\frac{1}{N_0}\Kprim_0(\mathbf{x}), \,\dots, \frac{1}{N_{Q-1}}\Kprim_{Q-1}(\mathbf{x}) \right]. \label{eq:ftm:9}
\end{align}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Relation between FTM and FNO-derived RNN Structures}
\label{subsec:fnoftm}

The FTM formulation allows some interpretation of the fast convolution layer proposed previously. The state equation \eqref{eq:ftm:7} describes the time-evolution of the modes phase and amplitude $\bar{\mathbf{y}}$. The state transition matrix $\mathrm{e}^{\As T}$ is diagonal, such that time-evolution of each mode state $\bar{\mathbf{y}}$ is decoupled. \eqref{eq:ftm:8} relates the mode states to the spatial variables $\mathbf{y}[\mathbf{x},k]$ by transformation matrix $\Cs(\mathbf{x})$. For geometrically simple examples, such as strings and rectangles, the underlying basis functions $\Kprim_\mu$ are trigonometric.

For a linear time-invariant system, the internal modes can be recovered readily from the spatial variable. The spatial variable transition matrix $\mathbf{S}$ for a discrete time step is defined by
\begin{align}
\mathbf{y}[\mathbf{x}_1,k+1] &= \mathbf{S}(\mathbf{x}_1,\mathbf{x}_2) \mathbf{y}[\mathbf{x}_2,k],
\label{eq:poles:1}
\end{align}
where the eigenvalue decomposition is
\begin{align}
    \mathbf{S}(\mathbf{x}_1,\mathbf{x}_2) = \Cs(\mathbf{x}_1) \mathrm{e}^{\As T} \Cs(\mathbf{x}_2)^{\dagger}.
\end{align}
\seb{I'm aware that this might not be proper notation here. Any better idea?} Transition matrix $\mathbf{S}$ can be numerically recovered from the spatial variables by solving a least squares in \eqref{eq:poles:1} on a sufficiently long time frame.

Similar operations are performed by the fast convolution layer. An FFT transforms the spatial variables into a transform domain where the basis functions are complex exponentials, thus also trigonometric functions. The processing step in \eqref{eq:fftlayer} applies a diagonal transition matrix $A_{ijk\hdots}$ to the transform-domain variables. The result is transformed back to the spatial variables via the inverse FFT.

There are also notable differences between the given approaches. The fast convolution layer applies a bias term. The NNs typically concatenates multiple layers and uses non-linear activation functions in-between. Because of the mapping performed by the first and last network layers, the NN is free to recombine and expand the spatial variable inputs and outputs.
